Specification of MiniDemographicABM.jl: A simplified agent-based demographic model of the UK

This documentation specifies a simplified non-calibrated demographic agent-based model of the UK, a largely simplified version of the Lone Parent Model presented in [Gostolil and Silverman 2020]. In the presented model, individuals of an initial population are subject to ageing, deaths, births, divorces and marriages throughout a simplified map of towns of the UK. The specification employs the formal terminology presented in [Elsheikh 2023a]. The main purpose of the model is to explore and exploit capabilities of the state-of-the-art Agents.jl Julia package [Datseris2022] in the context of demographic modeling applications. Implementation is provided via the Julia package MiniDemographicABM.jl [Elsheikh 2023b]. A specific simulation is progressed with a user-defined simulation fixed step size on a hourly, daily, weekly, monthly basis or even an arbitrary user-defined clock rate. The model can serve for comparative studies if implemented in other agent-based modelling frameworks and programming languages. Moreover, the model serves as a base implementation to be adjusted to realistic large-scale socio-economics, pandemics or immigration studies mainly within a demographic context.

==> 09outlook.tex <==
\section{Outlook}
\label{sec:outlook}


Significant population-oriented assumptions are formalized as follows:



%\begin{popass}
\graypopass{
\label{ass:pop:demographicEvents} 
As implicitly expressed by the set of events $\mathcal{E}$, cf.\ Section \ref{sec:example:formalOverview}, major demographic events s.a.\ world wars or pandemics are not considered
%\end{popass}
}
\todo{Move this to events section}
%\footnote{Unless such events are integrated into the input data which is currently in the actual implementation of version 1.1 not the case}
%\end{enumerate}
%\footnote{which events are excluded depend also on the simulation parameters} 
\setvalue{\popassnum}{6}


\grayass{
\label{ass:mixed:noImmigration} (In- and out-) immigration to the country is not included: 
    \begin{align}
    \label{eq:ass:mixed:noImmigration}
    \text{ if }  p \in & P_{isAlive}^{t}   ~\implies~ \nonumber \\ & town(p^t) \in W  ~\text{ and } \nonumber \\ 
    & \left( pre(town(p^t)) \in W ~\text{ or }~ age(p^t) = 0 \right) ~\text{ and } \nonumber \\
    & \left( post(town(p^{t})) \in W ~\text{ or }~  \neg isAlive(post(p^{t}) \right) \\
    \text{ for } t_0 <  t  < t_{final} \nonumber 
    %\text{ if } p \in P_{isAlive}^{t'} 
    %& \text{ where }  t_0 < t' \leq t_{final} ~\implies~ \nonumber \\ 
    %& pre(town(p^{t'})) \in W \text{ and } town(p^{t'}) \in W
\end{align}
}


In this article \comment{Attempt to sell and advocate the presented model despite being a simplified one, why is it still useful to have such a representative model}, the presented terminology is illustrated and demonstrated based on a simple agent-based demographic model of the United Kingdom, intentionally simplified to a superficial level. 
The model is mathematically constructed based on major simplified abstraction from the informal description provided in [citation to LPM paper] \comment{Lone Parent Model citation} associated with the corresponding large-scale code repository implemented in the Python programming language. \\ 

The purpose of this simplification and abstraction is
to have a formal model that serves as  an illustrative example for
\begin{enumerate}
\item 
 a compact but powerful terminology for formal specification of such agent-based demographic models 
\item 
an initial implementation as a starting point to build upon when modeling and simulating a specific and sophisticated case study imposing large-scale demographic context 
\end{enumerate}

The first goal is the main contribution presented in this paper whereas the second goal has been largely 
accomplished 

depending on the context, (e.g.\ pandemics, Socio-economics, immigration, social care etc.), the existing building blocks of the simplified model (or new ones) can be subject to tuning and  modification or insertion) according to the process of model tuning. 
Tuning a pre-given model rather than building it from scratch towards a specific case study may provide the possibility to examine and justify whether a particular tuning step, e.g. enhancing further details, is justifiable possible with qualitative metrics s.a.\ model predictive power. \\ 

While successful appliance of software engineering techniques \comment{Citations to multiple dispatch and others, e.g. High-performance symbolic-numerics via multiple dispatch } shall enhance such incremental model development process, this is not claimed within the scope of this document since implementation details are out of the scope of this work. This remains a promising achievement out of the many future potential extensions based on this work. Namely, the introduced simplified model provides  opportunities to examine: 
%
\begin{itemize}
\item 
Existing state-of-the-art modeling frameworks
\item 
Existing state-of-the-art mathematical tools including but not limited to calibration, sensitivity analysis, stochastic analysis and other mathematical tools for model-based applications among others
\item 
Machine learning based applications s.a.\ surrogate modeling 
\item 
Infrastructure tools for visualization and cloud computing 
\end{itemize}


\subsection*{Materials}

Nevertheless, based on this work, the authors are \comment{probably this paragraph belongs to Outlook} particularly targeting the employment of existing state-of-the-art packages provided in the Julia language. The aim is to identify the overall advantages and the shortages of the Julia-language ecosystem in the context of large-scale sophisticated demographic-based modeling applications. 
It is not desired to establish new tools or novel algorithms from scratch but rather to identify their tuning- or extension-potentials for the purpose of prototyping realistic sophisticated demographic models. 

==> _parameters_data.tex <==
\section{Parameters and input data} 
\label{sec:parametersdata}

\subsection{Parameters}
\label{sec:parametersdata:parameters}



\subsubsection{Model parameters}
\label{sec:parameters:modelpar}

\input{_parameters}

\subsection{Data}
\label{sec:parametersdata:data}

\input{_data}


==> casestudies.tex <==
\section{Potential case studies}
\label{sec:casestudies}

\subsection{Proposed initial populations} 

Potential forms of initial populations (i.e.\ the distribution of ages etc., i.e. young population, intermediate , old etc.)  
% 
\begin{center}
%\begin{tabular}{ |p{50mm}|p{50mm}| }
\begin{tabular}{ |l|l| }
\hline
Initial population & Potential practical extensions \\  
\hline 
Simplified demography dynamics & Social care \\  
\hline 
&  \\ 
\hline 
&   \\ 
\hline
\end{tabular}
\end{center}


\subsection{Proposed simulation parameters}

The following table proposes several case studies each comprises featured sub-populations associated with simulation parameters 
% 
\begin{center}
\begin{tabular}{ |l|c|c|c| } 
 \hline
 IPS & $t_0$ & $t_{final}$ & $\Delta t$ \\  
 \hline 
    $P_0 \in {10^3, 10^4, 10^5, 10^6}$  & 2010  & 2020 & Daily, Weekly or Monthly \\ 
\hline 
  &  &  &  \\ 
\hline 
 & &  &   \\ 
 \hline
\end{tabular}
\end{center}

==> paper01introduction.tex <==
\section{Introduction} 
\label{sec:introduction}


\subsection{Motivation}

\todo[inline]{Suggestion: Motivation that paves the way to why is it beneficial to have a formal terminology for specification for ABM in the field of social computational sciences}. \todo[inline]{An argumentation to sell the proposed terminology from social computational science  agent-based modeling perspective. 
}  

E.g. 
\begin{itemize}
    \item Informal model specification is ambiguous 
    \item Large-scale models need to be carried out by various scientists, modelers and developers each 
    \item Serve as a formal model documentation
    \item easier to detect dis-agreements 
\end{itemize}

I don't think that this paper should really consider argumentation regarding ODD's (this can be actually another paper), but still here are critical issues regarding ODD (This is in appendix) 
\begin{itemize}
    \item 
    The model specification is not following the ODD standard 
    \item 
    Standard gives the impression that ODD follows a formal pattern, though a significant portion of an ODD more or less constitutes of informal model description 
    \item 
    A standard should expresses an exact specification that is capable of replicating the same model using different frameworks and languages where as ODD rather focuses on information exchange and communication among domain experts and modelers and therefore the correctness is not guaranteed 
    \item 
    hence there is no guarantee that what is being described in an ODD is actually what is being implemented 
    \item
    On the other hand 
    a Modelica model (and ModelingToolkit.jl likewise) is an exact specification of a mathematical model that can be simulated as well
    \item 
    The proposed terminology is not suggested as an alternative for ODD but actually it could be integrated into ODD concept, in order to inspire solutions for the existing challenges. However, explicit suggestions are out of the scope of this work \comment{An outlook}
    \item the limited availability of guidance on how to use ODD
    \item limitations of ODD for highly complex models
    \item and the lack of provision for sections in the document structure covering model design rationale, the model’s underlying narrative, and the means by which the model’s fitness for purpose is evaluated
    \item  lack of sufficient details of many ODDs to enable re-implementation without access to the model code;
    \item simply different goals are served 
    \item The current model does not address emergent properties 
    \item It is quite an overhead to write an ODD especially if the implementation of the model, whether with NetLogo, Python or Agents.jl, is well-structured and well-documented following common software engineering techniques regarding coding guidelines, source file documentation, code structuring, design patterns, unit testing among others     
    \item 
    It seems that everyone who writes an O.D.D.\ would suggest a further update or modification to its contents  
\end{itemize}


\todo[inline]{Further improve what the contribution is about}

\subsection{Contribution}

This contribution is primarily concerned with proposing a novel terminology for specifying the mathematical description of agent-based models within a demographic context. 
% 
Particularly, a formal description of fixed-step single-clocked simulation process is presented. 
% 
It is assumed that
\begin{itemize}
    \item all agents are simultaneously progressed according to a \textit{single clock} 
    \item the time clock is progressed along \textit{fixed-step size}
    \item there is no subgroup of agents or subsystems subject to their own clock
\end{itemize} 
The terminology does not span multi-agents models (i.e.\ model with multiple types of agents), though it enables the specification of (or subgroups of agents, i.e.\ a single-level sub-population), cf.\  citation \comment{Citation to a multilevel-modeling Eric paper / Book} for the concept of multi-level agent-based models which is beyond the scope of this work. \\ 

The proposed terminology is illustrated and demonstrated on a simplified demographic model targeting agent-based simulation processes. 
The example model is a simplified version of the model presented in X \comment{Citation to the LPM} concerned with evaluating the impact of social care policies in the UK on social care demand in a socio-economic context. \\

As highlighted in Section \ref{sec:outlook}, the example model has been implemented in the Julia language using state-of-the-art agent-based modeling package Agents.jl \comment{citation to Agents.jl} and enhanced with a decent set of unit tests for effective incremental programming \comment{reference incremental programming / extreme programming}.  
%
The code is published within the model code base following FAIR principles \comment{citation} and is citable according to recommended software citations principles \comment{citation to MiniDemographicABM.jl}. 
%
Nevertheless, this contribution neither favors a particular programming language nor proposes particular agent-based modeling frameworks. While the presented model can actually serve as base model for comparative studies among programming langauges and modeling libraries, implementation-details are out of the scope of this work. \\

The rest of the work is structured as follows. Section \ref{sec:terminology} introduces the fundamental terminologies employed throughout this contribution. 
% 
Section \ref{sec:temporal} proposes a set of temporal operators, inspired by temporal logic \comment{reference}, with which sophisticated phrases can be algorithmically specified in a simple and compact manner.     
% 
Section \ref{sec:generalform} formulates a general specification of agent-based models and their simulation processes.  
% 
The proposed formal specification is then illustrated throughout a simplified demographic model informally introduced in Section \ref{sec:examplemodel} together with a list of simplification assumptions. 
% 
Afterwords, more detailed insights into the model space on which agents are operating is given in Section \ref{sec:space}.  
Subsequently, the set of model events influencing the states of agents is specified in Section \ref{sec:events}. 
Finally, section \ref{sec:outlook} provides further insights into the implementation of the demonstrated model and the aims behind. 



==> paper062space.tex <==
\subsection{Space $S$}
\label{sec:generalform:space}


A possible space can be to set as: 
% 
\begin{equation}
\label{eq:space}
S(t) = <H(t),W> 
\end{equation}
%
composed of a tuple of the set of houses $H(t)$ distributed within the set of towns $W$. 
Here is the set of towns are meant to be 

Resoundingly from Section \ref{sec:general:definitions}, the space $ S $ is composed of a tuple 
$$S ~\equiv~ S(t) ~=~ <H(t)~,~W> $$ corresponding to the set of all houses $H(t)$ and towns $W$ implying that: 
\begin{enumerate}[label=\textbf{S. \arabic*}]
\item 
the space is not necessarily static and particularly the set of houses can vary along the simulation time span 
\item \label{ass:space:staticTowns} the set of towns is constant during a simulation, i.e.\ no town vanishes nor new ones get constructed 
\item 
each town $w \in W$ contains a dynamic set of of houses $H_w \equiv H_w(t)$ 
\end{enumerate}
Furthermore,
\begin{enumerate}[label=\textbf{S. \arabic*}]
\setItemnumber{4}
\item 
each house $h \in H(t)$ is located in one and only one town $w \in W$, i.e. 
$$town(h) = w \in W$$ 
\item 
the location of each house $h \in H_w$ is given in xy-coordinate of the town
$$location(h_{x,y} \in H_w) = (x,y)_w$$
\item 
\label{ass:space:housingUniformLocations}
the houses within a town are uniformly distributed along the x and y axes
\item 
\label{ass:space:inhabitable}
a house never get demolished and remains always inhabitable 
\end{enumerate} 


==> paper06example.tex <==
\section{Model example}
\label{sec:examplemodel}
\label{sec:assumptions}

In this Section, snippets of a model example documented and implemented in \cite{MiniDemographicABMjlMisc} are briefly presented to demonstrate the descriptive capabilities of the proposed formal terminology.

\input{paper061overview}

